DepthTrack : Unveiling the Power of RGBD Tracking

RGBD (RGB plus depth) object tracking is gaining momentum as RGBD sensors have become popular in many application fields such as robotics.However, the best RGBD trackers are extensions of the state-of-the-art deep RGB trackers. They are trained with RGB data and the depth channel is used as a sidekick for subtleties such as occlusion detection. This can be explained by the fact that there are no sufficiently large RGBD datasets to 1) train deep depth trackers and to 2) challenge RGB trackers with sequences for which the depth cue is essential. This work introduces a new RGBD tracking dataset - Depth-Track - that has twice as many sequences (200) and scene types (40) than in the largest existing dataset, and three times more objects (90). In addition, the average length of the sequences (1473), the number of deformable objects (16) and the number of annotated tracking attributes (15) have been increased. Furthermore, by running the SotA RGB and RGBD trackers on DepthTrack, we propose a new RGBD tracking baseline, namely DeT, which reveals that deep RGBD tracking indeed benefits from genuine training data. The code and dataset is available at https://github.com/xiaozai/DeT

==> fig/fig_DeT_ATOM.tex <==
\begin{figure}[h]
\centering

    \begin{subfigure}[b]{0.8\linewidth}
         \centering
         \includegraphics[width=\textwidth]{fig/img/figure_for_trainable_rgbd_tracker_ATOM.png}
        %  \caption{The architecture of the variant DeT-ATOM, and the merging types include the convolutional layer, the element-wise maximum and mean operations.}
        \caption{DeT-ATOM}
         \label{fig:DeT_ATOM}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.8\linewidth}
         \centering
         \includegraphics[width=\textwidth]{fig/img/figure_for_trainable_rgbd_tracker_DiMP50.png}
        %  \caption{The architecture of the variant DeT-DiMP50, and the merging types include the convolutional layer, the element-wise maximum and mean operations.}
        \caption{DeT-DiMP50}
         \label{fig:DeT_DiMP50}
     \end{subfigure}
    \caption{The architectures of the DeT variants.}%, and the merging types include the convolutional layer, the element-wise maximum and mean operations.}

% \includegraphics[width=0.75\linewidth]{fig/img/figure_for_trainable_rgbd_tracker_ATOM.png}
% %\vspace{-0.2cm}
% \caption{
% % \caption{The head part of the proposed DeT RGBD tracker. The tail part
% % depends on the selected architecture (e.g. ATOM or DiMP) and can be changed.
% % $F$-s are the backbone networks (e.g. ResNet), but in our case the
% % D backbone branch is trained from scratch with depth
% % tracking data and thus unveils the power of depth for tracking.
% The architecture of the variant DeT-ATOM, and the merging types include the convolutional layer, the element-wise maximum and mean operations.
% %The deep RGB and depth feature maps are extracted by two feature extractors , $F_{rgb}$ and $F_{depth}$, from the input frames,
% %and then are concatenated along the channels.
% %The merge operation can be 1) a convolutional layer with $1\times1$ kernel size, 2) the element-wise maximum operation or 3) the element-wise mean operation, which merges the feature maps at each pixel position.
% %The fused feature maps $D_{rgbd}$ are then fed into the following tracking modules.
% }

% \label{fig:DeT_ATOM}
\end{figure} 

==> fig/fig_DeT_DiMP50.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.75\linewidth]{fig/img/figure_for_trainable_rgbd_tracker_DiMP50.png}
%\vspace{-0.2cm}
\caption{
% \caption{The head part of the proposed DeT RGBD tracker. The tail part
% depends on the selected architecture (e.g. ATOM or DiMP) and can be changed.
% $F$-s are the backbone networks (e.g. ResNet), but in our case the
% D backbone branch is trained from scratch with depth
% tracking data and thus unveils the power of depth for tracking.
The architecture of the variant DeT-DiMP50, and the merging types include the convolutional layer, the element-wise maximum and mean operations.
%The deep RGB and depth feature maps are extracted by two feature extractors , $F_{rgb}$ and $F_{depth}$, from the input frames,
%and then are concatenated along the channels.
%The merge operation can be 1) a convolutional layer with $1\times1$ kernel size, 2) the element-wise maximum operation or 3) the element-wise mean operation, which merges the feature maps at each pixel position.
%The fused feature maps $D_{rgbd}$ are then fed into the following tracking modules.
}
\label{fig:DeT_DiMP50}
\end{figure*} 

==> fig/fig_attributes_distribution.tex <==
\begin{figure}
\centering
\includegraphics[width=0.95\linewidth]{fig/img/fig_for_dataset_attribute_distribution.png}
\caption{The number of frames for visual attributes in the DepthTrack test set.
Number denotes the number of frames.}
\label{fig:fig_attributes_distribution}
\end{figure}                                 


==> fig/fig_fscores_over_attributes.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=0.99\linewidth]{fig/img/fig_for_attribute_fscores.png}
    \caption{
    \song{Song:TOO MANY COLOR!!!} Optimal F-Score average over overlap thresholds for the visual attributes.
    Stars denotes the best F-score over attributes achieved by the corresponding trackers. The abbreviation for each attribute is as follows: aspect change (AC), background clutter (BC), depth change (DC), fast motion (FM), dark scene (DS), full occlusion (FO), camera motion (CM), non-rigid deformation (ND), out of plane (OP), out of frame (OF), partial occlusion (PO), reflective targets (RT), size change (SC), similar objects (SO) and unassigned (NaN).}
    \label{fig:attribute_fscores}
\end{figure*}

==> fig/fig_fscores_over_attributes_CDTB.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{fig/img/fig_for_attribute_fscores_CDTB.png}
    \caption{Optimal F-scores %which is the average over overlap thresholds 
    for the visual attributes on CDTB dataset~\cite{Lukezic_2019_ICCV}.
    % Stars denotes the best F-score over attributes achieved by the corresponding trackers. 
    % The abbreviation for each attribute is as follows: aspect change (AC), background clutter (BC), depth change (DC), fast motion (FM), dark scene (DS), full occlusion (FO), camera motion (CM), non-rigid deformation (ND), out of plane (OP), out of frame (OF), partial occlusion (PO), reflective targets (RT), size change (SC), similar objects (SO) and unassigned (NaN).
    ATOM and its variants perform very similar on the \textit{out-of-frame} (OF) attribute.
    }
    \label{fig:attribute_fscores_CDTB}
\end{figure}

==> fig/fig_pr_re_fscores.tex <==
\begin{figure*}[h]
\centering
\includegraphics[width=0.99\linewidth]{fig/img/fig_for_pr-re-fscores.png}
\caption{The Precision-Recall and F-score curves of the evaluated trackers (the best F-score point marked in each graph). Left: sequence-based; Right: frame-based evaluation.}
\label{fig:fig_trackers_pr_re_fscore_final_all}
\end{figure*}    

==> fig/fig_qualititative_evaluation_CDTB.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.75\linewidth]{fig/img/fig_for_qualitative_experiments_CDTB.png}
\caption{
Examples from the CDTB benchmark (targets marked with white boxes in depth images):
similar background color (1st row),
single targets (2nd row),
wild scenes (3rd row),
glasses (4th row),
dark scenes (5th row),
long boxes (6th row),
depth missing scenes (7th row).
% failure cases (8th row).
In addition to the existing baselines, the DeT-DiMP50-Max and DeT-ATOM-Max outputs are marked in the depth images.}
\label{fig:qualitative-evaluation-cdtb}
\end{figure*} 

==> tbl/fscores_on_each_sequences.tex <==
\begin{table}[]
\label{fscores_on_each_seq}
    \centering
    \begin{tabular}{c| c c c c c c}
        Sequence          & DiMP50 & DeT-DiMP50-DO & DeT-DiMP50-Max & ATOM    & DeT-ATOM-MC & DeT-ATOM-Max \\
        adapter01\_indoor & 0.599  & ~             & 0.711          & 0.652   & 0.709       &              \\
        backpack\_indoor  & 0.188  & ~             & 0.222          & 0.304   & 0.269       &              \\
        bag01\_indoor     & 0.050  & ~             & 0.698          & 0.061   & 0.702       &              \\
        bag02\_indoor     & 0.042  & ~             & 0.264          & 0.025   & 0.149       &              \\
        ball01\_wild      & 0.112  & ~             & 0.663          & 0.491   & 0.569       &              \\
        ball06\_indoor    & 0.458  & ~             & 0.458          & 0.480   & 0.187       &              \\
        ball10_wild       & 0.303  & ~             & 0.181          & 0.029   & 0.237       &               \\
        ball11_wild 
        ball15_wild 
        ball18_indoor 
        ball20_indoor 
        bandlight_indoor 
        beautifullight02_indoor 
        book03_indoor 
        bottle04_indoor 
        card_indoor 
        cat01_indoor 
        colacan03_indoor 
        cube02_indoor 
        cude03_indoor 
        cube05_indoor 
        cup01_indoor 
        cup02_indoor 
        cup04_indoor 
        cup12_indoor 
        developmentboard_indoor 
        duck03_wild 
        dumbbell01_indoor 
        earphone01_indoor 
        file01_indoor 
        flag_indoor 
        glass01_indoor 
        hand01_indoor 
        human02_indoor 
        lock_wild 
        mobilephone03_indoor 
        notebook01_indoor 
        pigeon01_wild
        pigeon02_wild 
        pigeon04_wild 
        pot_indoor 
        roller_indoor
        shoes02_indoor 
        squirrel_wild 
        stick_indoor 
        toiletpaper01_indoor 
        toy02_indoor 
        toy09_indoor 
        ukulele01_indoor 
        yogurt_indoor 
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}

==> tbl/tbl_attribute.tex <==
% Please add the following required packages to your document preamble:
\newcolumntype{C}{>{\centering\arraybackslash}X}
\begin{table*}[h]
\begin{center}
\caption{
Tracking visual attributes including 10 manually annotated attributes and 5 ones calculated from the groundtruth.
}
\label{tbl:attribute}
\footnotesize
\resizebox{0.92\linewidth}{!}{%
\setlength\tabcolsep{1.5pt} % default value: 6pt
% \begin{tabularx}{\linewidth}{p{4cm} | p{1cm} | p{12cm} | C{1cm} }

\begin{tabularx}{0.99\linewidth}{l | c | l | c}
\toprule
\multicolumn{1}{c|}{Attribute} & Tag & \multicolumn{1}{c|}{Description} & Annotation\\
\midrule
\shortstack[c]{Aspect-ratio} Change & AC & When the ratio between maximum and minimum target size in 21 consecutive frames was larger than 1.5. & Calculated\\
Background Clutter & BC & Background near the target has the similar appearance as the target. & Manually\\
Camera Motion & CM & The camera view is not fixed. & Manually\\
Dark Scene & DS & No visible light is in the scenario. & Manually\\
% Depth Change & DC & \shortstack[l]{The ratio between maximum and minimum of median of depth within target region in 21 consecutive frames\\ was larger than 1.5.} & Automation\\
Depth Change & DC & \shortstack[l]{The ratio between maximum and minimum of depth median in target region in 21 frames was larger than 1.5.} & Calculated\\
Fast Motion & FM & The target center moves by at least 30\% of its size in consecutive frames. & Calculated\\
Full Occlusion & FO & The target is fully occluded. & Manually\\
%\textcolor{red}{Illumination Variation} & IV & The illumination in the target region is significantly changed. & Manually\\
% Motion Blur & MB & The target region is blurred due to the motion of target or camera.\\
Non-rigid Deformation & ND & The non-rigid object deforms. & Manually\\
Out-of-plane Rotation & OP & Target rotates out of the plane. & Manually\\
Out-of-frame & OF & Partial or the whole target leaves the view. & Manually\\
Partial Occlusion & PO & The target is partially occluded. & Manually\\
Reflective Targets & RT & Interface of the target is reflective. & Manually\\
Size Change & SC & When the ratio between maximum and minimum target size in 21 consecutive frames is larger than 1.5. & Calculated\\
Similar Objects & SO & There is adjacent objects whose appearance is similar to the target. & Manually\\
Unassigned & NaN & There is no aforementioned cases appeared in the frame. & Calculated\\

% \midrule
% Baseline   & - & - & - & LT & RGBD\\
\bottomrule
\end{tabularx}%
}
\end{center}
\end{table*}







% % Please add the following required packages to your document preamble:
% \newcolumntype{C}{>{\centering\arraybackslash}X}
% \begin{table}
% \begin{center}
% \caption{
% Attribute}
% \label{tbl:attribute}
% \resizebox{0.9\linewidth}{!}{%
% \begin{tabularx}{\linewidth}{p{2cm} | p{1cm} | p{5cm}}
% \toprule
% Attribute & Code & Description \\
% \midrule
% Aspect \textcolor{ratio} Change & AC & When the ratio between maximum and minimum target size in 21 consecutive frames was larger than 1.5.\\
% Background Clutter & BC & Background near the target has the similar appearance as the target. \\
% Dark Scene & DS & No visible light is in the scenario.\\
% Depth Change & DC & The ratio between maximum and minimum of median of depth within target region in 21 consecutive frames was larger than 1.5.\\
% Fast Motion & FM & The target center moves by at least 30\% of its size in consecutive frames.\\
% Full Occlusion & FO & The target is fully occluded.\\
% Illumination Variation & IV & The illumination in the target region is significantly changed.\\
% Moving View & MV & The camera view is not fixed.\\
% Non-rigid Deformation & ND & The non-rigid object deforms.\\
% Out-of-plane Rotation & OP & Target rotates out of the plane.\\
% Out of View & OV & Partial or the whole target leaves the view.\\
% Partial Occlusion & PO & The target is partially occluded.\\
% Reflective Targets & RT & Interface of the target is reflective.\\
% Size Change & SC & When the ratio between maximum and minimum target size in 21 consecutive frames is larger than 1.5.\\
% Similar Objects & SO & There is adjacent objects whose appearance is similar to the target.\\
% Unassigned & NaN & There is no aforementioned cases appeared in the frame.\\
% \bottomrule
% \end{tabularx}%
% }
% \end{center}
% \end{table}


==> tbl/tbl_experiments_trainable_trackers_on_CDTB.tex <==

\newcolumntype{C}{>{\centering\arraybackslash}X}
\begin{table*}[t]
\begin{center}
\caption{
Evaluation results of the trainable RGB and RGBD trackers on the CDTB benchmark.
}
\label{tbl:experiments_trainable_trackers_on_CDTB}
\small
\setlength\tabcolsep{4.5pt} % default value: 6pt
\resizebox{0.9\linewidth}{!}{%
\begin{tabularx}{\linewidth}{l | r r r | r r r | r | c c c c}
\toprule
~        & \multicolumn{3}{c|}{Sequence-based} & \multicolumn{3}{c|}{Frame-based}  & \multicolumn{1}{c|}{Speed} & \multicolumn{4}{c}{Training Datasets} \\
% 
Tracker  & \multicolumn{1}{c}{Pr} &\multicolumn{1}{c}{Re} & \multicolumn{1}{c|}{F-score} & \multicolumn{1}{c}{Pr} &\multicolumn{1}{c}{Re} & \multicolumn{1}{c|}{F-score} & \multicolumn{1}{c|}{fps} &  \multicolumn{1}{c}{Inputs}  & \multicolumn{1}{c}{RGB Datasets} & \multicolumn{1}{c}{Synthetic Depth} & \multicolumn{1}{c}{DepthTrack}  \\
\midrule
DiMP50~\cite{bhat2019learning}  &  0.549  & 0.555  & 0.552   & 0.546     & 0.549     &  0.547    & 55.39     &  RGB  & \checkmark & ~          & ~ \\
DiMP50~\cite{bhat2019learning}  &  0.580  & 0.571  & 0.575  & 0.561     & 0.563     & 0.562     & 52.57     &  RGB  & \checkmark & ~          & \checkmark \\
% 
DeT-DiMP50-DO        &   0.491   &   0.476   &   0.484   & 0.480     & 0.481     & 0.481     & 57.35     &  D    &  & \checkmark & \checkmark \\
% 
DeT-DiMP50-MC       & 0.631   & 0.621   & 0.626   & 0.622     & 0.624    & 0.623     & 32.95     & RGBD  & \checkmark & \checkmark & \checkmark \\
%
%
DeT-DiMP50-Max         &  0.651  &   0.633   &   0.642   & 0.626     & 0.621    & 0.624    & 40.54     & RGBD  & \checkmark & \checkmark & \checkmark \\
%
DeT-DiMP50-Mean         & \bf{0.674}   & \bf{0.642}   &  \bf{0.657}   & \bf{0.664}     & \bf{0.644}     & \bf{0.654}     & 42.76     & RGBD  & \checkmark & \checkmark & \checkmark \\

\midrule

ATOM~\cite{2019ATOM} &   0.548   &  0.536   &  0.542   &  0.541    &  0.537    &  0.539    & 55.43    & RGB   & \checkmark & ~          & ~ \\
% ATOM18~\cite{2019ATOM}            & -     & -     & -     & ~     & ~     & ~     & ~     & RGB  & \checkmark & ~          & \checkmark \\
% % 
% DeT-ATOM18-DO          &   -   &   -   &   -   & -     & -     & -     & -     &  D    & \checkmark & \checkmark & \checkmark \\
% % 
% DeT-ATOM-MC         &  \song{0.615}   &   0.599   &   0.607   & 0.615     & 0.593     & 0.604     & -    & RGBD  & \checkmark & \checkmark & \checkmark \\
DeT-ATOM-MC         &  0.582   &  0.567   &  0.574  & 0.572    & 0.574    & 0.573     & 45.98    & RGBD  & \checkmark & \checkmark & \checkmark \\
% %
DeT-ATOM-Max         &   -   &   -   &   -   & -     & -     & -     & -     & RGBD  & \checkmark & \checkmark & \checkmark \\
%
DeT-ATOM-Mean         &   -   &   -   &   -   & -     & -     & -     & -     & RGBD  & \checkmark & \checkmark & \checkmark \\


\bottomrule
\end{tabularx}%
}
\end{center}
\end{table*}

==> tbl/tbl_experiments_trainable_trackers_on_DepthTrack.tex <==

\newcolumntype{C}{>{\centering\arraybackslash}X}
\begin{table*}[t]
\begin{center}
\caption{
Evaluation results of the trainable RGB and RGBD trackers on the proposed DepthTrack test set, trackers are trained on the existing RGB benchmarks, the proposed estimated depth benchmarks and the training set of DepthTrack benchmark.
{\em RGB Datasets} include LaSOT~\cite{fan2019lasot}, TrackingNet~\cite{muller2018trackingnet}, GOT-10k~\cite{Huang_2019}, and COCO~\cite{lin2014microsoft} datasets, which are used for the SotA RGB trackers.
{\em Synthetic Depth} denotes the estimated depth images of LaSOT and COCO datasets.
{\em DepthTrack} denotes the training set of the DepthTrack benchmark.
{\em DeT-XXX} denotes the proposed RGBD trackers using DiMP50 or ATOM18 as the base tracker, 
"{\em -DO}" denotes the proposed depth-oriented tracker taking only the depth inputs.
"{\em-MC}" denotes merging the RGB and Depth deep features with the convolution operation,
while "{\em -Max}" denotes the element-wise maximum operation, 
and "{\em -Mean}" denotes the element-wise mean operation.
}
\label{tbl:experiments_trainable_trackers_on_DepthTrack}
\small
\setlength\tabcolsep{3.5pt} % default value: 6pt
\resizebox{0.9\linewidth}{!}{%
\begin{tabularx}{\linewidth}{l | r r r | r r r | r | c c c c}
\toprule
~        & \multicolumn{3}{c|}{Sequence-based} & \multicolumn{3}{c|}{Frame-based}  & \multicolumn{1}{c|}{Speed} & \multicolumn{4}{c}{Training Datasets} \\
% 
Tracker  & \multicolumn{1}{c}{Pr} &\multicolumn{1}{c}{Re} & \multicolumn{1}{c|}{F-score} & \multicolumn{1}{c}{Pr} &\multicolumn{1}{c}{Re} & \multicolumn{1}{c|}{F-score} & \multicolumn{1}{c|}{fps} &  \multicolumn{1}{c}{Inputs}  & \multicolumn{1}{c}{RGB Datasets} & \multicolumn{1}{c}{Synthetic Depth} & \multicolumn{1}{c}{DepthTrack}  \\
\midrule
DiMP50~\cite{bhat2019learning}  & 0.396 & 0.415 & 0.405 & 0.387 & 0.403 & 0.395 & 42.11 &  RGB  & \checkmark & ~    & ~ \\
DiMP50~\cite{bhat2019learning}  & 0.483 & 0.468 & 0.475 & 0.443     & 0.433     & 0.438     & 54.70     &  RGB  & \checkmark & ~    & \checkmark \\
DiMP50~\cite{bhat2019learning}  & 0.249 & 0.176 & 0.206 & 0.218     & 0.193     & 0.205     & 55.23     &  D    & \checkmark & ~    & ~ \\

% \hline

DeT-DiMP50-DO        & 0.266 & 0.233 & 0.248 & 0.250     & 0.244     & 0.247     & 48.51     &  D    & ~ & \checkmark & ~ \\
DeT-DiMP50-DO        & 0.396 & 0.339 & 0.365 & 0.379     & 0.351     & 0.364     & 56.07     &  D    &   & ~          & \checkmark \\
DeT-DiMP50-DO        & 0.412 & 0.377 & 0.394 & 0.423     & 0.400     & 0.411     & 59.01     &  D    &  & \checkmark & \checkmark \\

% \hline

DeT-DiMP50-MC       & 0.466 & 0.423 & 0.443 & 0.451     & 0.418     & 0.434     & 42.01     & RGBD  & \checkmark & \checkmark & ~ \\
DeT-DiMP50-MC       & 0.500 & 0.454 & 0.476 & 0.478     & 0.442     & 0.459     & 41.29     & RGBD  & \checkmark & ~          & \checkmark \\
DeT-DiMP50-MC       & 0.512 & 0.482 & 0.496 & 0.495    & 0.469     & 0.482    & 38.92     & RGBD  & \checkmark & \checkmark & \checkmark \\

%
DeT-DiMP50-Max     & - & - & - & - & - & - & - & RGBD & \checkmark & \checkmark & ~ \\
DeT-DiMP50-Max     & - & - & - & - & - & - & - & RGBD & \checkmark & ~ & \checkmark \\
DeT-DiMP50-Max     &   \bf{0.560} &  0.506  &   \bf{0.532}   & \bf{0.523}     & 0.479     & \bf{0.500}     & 36.88     & RGBD  & \checkmark & \checkmark & \checkmark \\
DeT-DiMP50-Mean    &  0.540   &  \bf{0.520}   &  0.530   & 0.508     & \bf{0.486}     & 0.497     & 41.23    & RGBD  & \checkmark & \checkmark & \checkmark \\

\midrule

ATOM~\cite{2019ATOM}            & 0.354 & 0.371 & 0.363 & 0.329 & 0.343 & 0.336 & 43.21 & RGB   & \checkmark & ~          & ~ \\
% ATOM~\cite{2019ATOM}            & -     & -     & -     & ~     & ~     & ~     & ~     & RGB  & \checkmark & ~          & \checkmark \\
% ATOM~\cite{2019ATOM}            &   -   &   -   &   -   & -     & -     & -     & -     & D    & \checkmark & ~          & ~ \\

% % \hline

% DeT-ATOM-DO        & -     & -     & -     & -     & -     & -     & -     &  D    & \checkmark & \checkmark & ~ \\
% DeT-ATOM-DO        &  -    &   -   &  -    & -     & -     & -     & -     &  D    & \checkmark & ~          & \checkmark \\
% DeT-ATOM-DO        &   -   &   -   &   -   & -     & -     & -     & -     &  D    & \checkmark & \checkmark & \checkmark \\

% % \hline

% DeT-ATOM-MC       & -     & -     & -     & -     & -     & -     & -     & RGBD  & \checkmark & \checkmark & ~ \\
% DeT-ATOM-MC       & -     & -     & -     & -     & -     & -     & -     & RGBD  & \checkmark & ~          & \checkmark \\
DeT-ATOM-MC         & 0.457 & 0.423 & 0.440 & 0.438 & 0.414 & 0.426    & 48.39    & RGBD  & \checkmark & \checkmark & \checkmark \\
DeT-ATOM-Max        & -     & -     & -     & -     & -     & -     & -     & RGBD  & \checkmark & \checkmark & \checkmark \\
DeT-ATOM-Mean       & -     & -     & -     & -     & -     & -     & -     & RGBD  & \checkmark & \checkmark & \checkmark \\

% %
% DeT-ATOM-Max       &   -   &   -   &   -   & -     & -     & -     & -     & RGBD  & \checkmark & \checkmark & \checkmark \\
% DeT-ATOM-Mean   &   -   &   -   &   -   & -     & -     & -     & -     & RGBD  & \checkmark & \checkmark & \checkmark \\

\bottomrule
\end{tabularx}%
}
\end{center}
\end{table*}

==> tbl/tbl_fscores_over_attributes.tex <==
% % Please add the following required packages to your document preamble:
% \newcolumntype{C}{>{\centering\arraybackslash}X}
% \begin{table*}[t]
% \begin{center}
% \caption{
% Optimal F-score averaged over overlap thresholds for the visual attributes.
% }
% \label{tbl:fscores_attributes_on_DeTrack}
% \resizebox{\linewidth}{!}{%
% % \begin{sidewaystable}
% \begin{tabularx}{0.95\linewidth}{l | r r r r r r r r r r r r r r r }
% \toprule
% Tracker &  AC & BC & DS & DC & FM & FO & MV & ND & OP & OV & PO & RT & SC & SO & NaN \\
% \midrule
% DDiMP      & 0.314756 & 0.377464 & 0.580357 & 0.377386 & 0.399759 & 0.474566 & 0.704594 & 0.632917 & 0.438265 & 0.487342 & 0.350532 & 0.643394 & 0.393287 & 0.479915 & 0.570401 \\
% ATCAIS     & 0.356642 & 0.406220 & 0.530372 & 0.380153 & 0.357932 & 0.499362 & 0.642443 & 0.562152 & 0.422056 & 0.499757 & 0.348573 & 0.647361 & 0.394137 & 0.450204 & 0.627060 \\

% CLGS\_D    & 0.288481 & 0.311975 & 0.367804 & 0.371127 & 0.354202 & 0.879356 & 0.778928 & 0.529604 & 0.405508 & 0.686681 & 0.374267 & 0.416250 & 0.323965 & 0.390653 & 0.574356 \\
% SiamDW\_D  & 0.272414 & 0.315821 & 0.408108 & 0.275900 & 0.339585 & 0.499375 & 0.739836 & 0.572064 & 0.377931 & 0.499773 & 0.353642 & 0.421063 & 0.304431 & 0.389265 & 0.533368 \\
% LTDSEd     & 0.257919 & 0.308781 & 0.388294 & 0.226506 & 0.311955 & 0.246288 & 0.714745 & 0.486866 & 0.351804 & 0.224153 & 0.297092 & 0.230103 & 0.275079 & 0.396853 & 0.482894 \\
% Siam\_LTD  & 0.193829 & 0.296616 & 0.262334 & 0.215674 & 0.226646 & 0.499337 & 0.617194 & 0.490947 & 0.308944 & 0.499742 & 0.226892 & 0.542607 & 0.212027 & 0.318239 & 0.490616 \\
% SiamM\_Ds  & 0.173840 & 0.237421 & 0.288879 & 0.210322 & 0.229805 & 0.499375 & 0.648641 & 0.528345 & 0.252665 & 0.499768 & 0.176764 & 0.006764 & 0.186518 & 0.318265 & 0.351159 \\
% \midrule
% DAL \cite{2019DAL} & 0.259456 & 0.354704 & 0.501333 & 0.316975 & 0.359452 & 0.489549 & 0.720490 & 0.551184 & 0.400263 & 0.492536 & 0.310564 & 0.191523 & 0.299441 & 0.443874 & 0.478429 \\
% CA3DMS      & 0.130549 & 0.248022 & 0.376734 & 0.124357 & 0.124646 & 0.0 & 0.308507 & 0.227354 & 0.237854 & 0.0 & 0.214617 & 0.088476 & 0.155384 & 0.195366 & 0.265416 \\
% DS-KCF & 0.043141 & 0.057095 & 0.046745 & 0.044573 & 0.021305 & 0.0 & 0.068575 & 0.083313 & 0.062978 & 0.0 & 0.090019 & 0.029056 & 0.042501 & 0.118233 & 0.088737 \\
% DS-KCF-Shape & 0.044319 & 0.059766 & 0.048071 & 0.041559 & 0.024453 & 0.0 & 0.075537 & 0.084089 & 0.060233 & 0.0 & 0.084546 & 0.038313 & 0.040734 & 0.104406 & 0.069404 \\
% \midrule
% LTMU\_B    & 0.309598 & 0.377457 & 0.467020 & 0.346851 & 0.416346 & 0.494426 & 0.753923 & 0.564227 & 0.427045 & 0.497117 & 0.337744 & 0.456076 & 0.366336 & 0.519358 & 0.495145 \\
% RLT\_DiMP  & 0.311287 & 0.404120 & 0.593991 & 0.366407 & 0.429500 & 0.207876 & 0.735952 & 0.598446 & 0.419880 & 0.239406 & 0.323849 & 0.659889 & 0.361927 & 0.449620 & 0.502586 \\
% Megtrack   & 0.259406 & 0.296357 & 0.364473 & 0.247500 & 0.325000 & 0.099796 & 0.738276 & 0.542998 & 0.376838 & 0.243113 & 0.306950 & 0.439949 & 0.289506 & 0.365891 & 0.536395 \\
% \midrule
% PrDiMP50   & 0.275623 & 0.321849 & 0.210337 & 0.282180 & 0.370113 & 0.0 & 0.714927 & 0.551652 & 0.384117 & 0.0 & 0.321316 & 0.376384 & 0.323473 & 0.461162 & 0.420400 \\
% DiMP50     & 0.257859 & 0.319690 & 0.295264 & 0.296599 & 0.391397 & 0.0 & 0.665336 & 0.524933 & 0.339592 & 0.0 & 0.254847 & 0.549704 & 0.309004 & 0.434979 & 0.428401 \\
% ATOM       & 0.207213 & 0.282452 & 0.273717 & 0.250177 & 0.270326 & 0.0 & 0.684066 & 0.514768 & 0.287907 & 0.0 & 0.281734 & 0.531974 & 0.231880 & 0.353278 & 0.308396 \\
% SiamRPN    & 0.198147 & 0.226873 & 0.351586 & 0.241806 & 0.221974 & 0.370867 & 0.655433 & 0.494361 & 0.311542 & 0.439775 & 0.217435 & 0.557400 & 0.214252 & 0.285505 & 0.402504 \\
% D3S        & 0.140946 & 0.198315 & 0.257385 & 0.203502 & 0.138251 & 0.0 &  0.498767 & 0.418112 & 0.244550 & 0.0 & 0.249963 & 0.418031 & 0.177375 & 0.254718 & 0.272649 \\
% SiamFC     & 0.099343 & 0.161730 & 0.153023 & 0.117383 & 0.089878 & 0.0 & 0.279496 & 0.339293 & 0.152883 & 0.0 & 0.118539 & 0.183943 & 0.104192 & 0.177431 & 0.224180 \\
% \midrule
% AlphaRef   & 0.376530 & 0.399319 & 0.342998 & 0.399464 & 0.376079 & 0.0 & 0.720163 & 0.608733 & 0.492745 & 0.0 & 0.343739 & 0.414390 & 0.372472 & 0.396323 & 0.549598 \\
% RPT        & 0.300828 & 0.326231 & 0.188928 & 0.306576 & 0.276930 & 0.499375 & 0.603405 & 0.548581 & 0.367257 & 0.499773 & 0.299684 & 0.456857 & 0.297611 & 0.326830 & 0.494513 \\
% OceanPlus  & 0.245622 & 0.297097 & 0.256224 & 0.229823 & 0.237374 & 0.499349 & 0.697014 & 0.527568 & 0.345849 & 0.499752 & 0.259048 & 0.535306 & 0.247090 & 0.318463 & 0.420722 \\
% % \midrule
% % Baseline   & - & - & - & LT & RGBD\\
% \bottomrule
% \end{tabularx}%
% }
% % \end{sidewaystable}
% \end{center}
% \end{table*}

% Please add the following required packages to your document preamble:
\newcolumntype{C}{>{\centering\arraybackslash}X}
\begin{table*}[t]
\begin{center}
\caption{
Optimal F-score averaged over overlap thresholds for the visual attributes.
}
\label{tbl:fscores_attributes_on_DeTrack}
\resizebox{0.95\linewidth}{!}{%
% \begin{sidewaystable}
\footnotesize
\setlength\tabcolsep{3.6pt} % default value: 6pt
\begin{tabularx}{1.02\linewidth}{l | c c c c c c c c c c c c c c c }
\toprule
Tracker                             &  AC    & BC          & DS     & DC     & FM     & FO     & CM     & ND     & OP     & OF     & PO     & RT     & SC             & SO     & NaN \\
\midrule
DDiMP \cite{Kristan2020a}           & 0.3148 & 0.3774      & 0.5804 & 0.3774 & 0.3998 & 0.4746 & 0.7046 & \textbf{0.6329} & 0.4383 & 0.4873 & 0.3505 & 0.6434 & 0.3933 & 0.4799 & 0.5704 \\
ATCAIS \cite{Kristan2020a}          & 0.3566 & \bf{0.4062} & 0.5304 & 0.3802 & 0.3579 & 0.4994 & 0.6424 & 0.5622 & 0.4221 & 0.4998 & 0.3486 & 0.6474 & \textbf{0.3941} & 0.4502 & \textbf{0.6271} \\
CLGS\_D \cite{Kristan2020a}         & 0.2885 & 0.3120      & 0.3678 & 0.3711 & 0.3542 & \textbf{0.8794} & \textbf{0.7789} & 0.5296 & 0.4055 & \textbf{0.6867} & \textbf{0.3743} & 0.4163 & 0.3240 & 0.3907 & 0.5744 \\
SiamDW\_D                           & 0.2724      & 0.3158      & 0.4081 & 0.2759 & 0.3396 & 0.4994 & 0.7398 & 0.5721 & 0.3779 & 0.4998 & 0.3536 & 0.4211 & 0.3044 & 0.3893 & 0.5334 \\
LTDSEd \cite{kristan2019seventh}    & 0.2579      & 0.3088      & 0.3883 & 0.2265 & 0.3120 & 0.2463 & 0.7147 & 0.4869 & 0.3518 & 0.2242 & 0.2971 & 0.2301 & 0.2751 & 0.3969 & 0.4829 \\
Siam\_LTD \cite{Kristan2020a}       & 0.1938      & 0.2966      & 0.2623 & 0.2157 & 0.2266 & 0.4993 & 0.6172 & 0.4909 & 0.3089 & 0.4997 & 0.2269 & 0.5426 & 0.2120 & 0.3182 & 0.4906 \\
SiamM\_Ds \cite{kristan2019seventh} & 0.1738      & 0.2374      & 0.2889 & 0.2103 & 0.2298 & 0.4994 & 0.6486 & 0.5283 & 0.2527 & 0.4998 & 0.1768 & 0.0068 & 0.1865 & 0.3183 & 0.3512 \\
\midrule
DAL \cite{2019DAL}                  & 0.2595      & 0.3547      & 0.5013 & 0.3170 & 0.3595 & 0.4895 & 0.7205 & 0.5512 & 0.4003 & 0.4925 & 0.3106 & 0.1915 & 0.2994 & 0.4439 & 0.4784 \\
CA3DMS \cite{liu2018context}        & 0.1305      & 0.2480      & 0.3767 & 0.1244 & 0.1246 & 0.2569 & 0.3085 & 0.2274 & 0.2379 & 0.2314 & 0.2146 & 0.0885 & 0.1554 & 0.1954 & 0.2654 \\
DS-KCF \cite{camplani2015real}      & 0.0431      & 0.0571      & 0.0467 & 0.0446 & 0.0213 & 0.0 & 0.0686 & 0.0833 & 0.0630 & 0.0 & 0.0900 & 0.0296 & 0.0425 & 0.1182 & 0.0887 \\
DS-KCF-Shape \cite{2016DS}          & 0.0443      & 0.0598      & 0.0481 & 0.0416 & 0.0245 & 0.0 & 0.0755 & 0.0841 & 0.0602 & 0.0103 & 0.0845 & 0.0383 & 0.0407 & 0.1044 & 0.0694 \\
\midrule
LTMU\_B \cite{Kristan2020a}         & 0.3096      & 0.3775      & 0.4670 & 0.3469 & 0.4163 & 0.4944 & 0.7539 & 0.5642 & 0.4270 & 0.4971 & 0.3377 & 0.4561 & 0.3663 & \textbf{0.5194} & 0.4951 \\
RLT\_DiMP \cite{Kristan2020a}       & 0.3113      & 0.4041      & \bf{0.5940} & 0.3664 & \bf{0.4295} & 0.2079 & 0.7360 & 0.5984 & 0.4199 & 0.2394 & 0.3238 & \textbf{0.6599} & 0.3619 & 0.4496 & 0.5026 \\
Megtrack \cite{Kristan2020a}        & 0.2594      & 0.2964      & 0.3645 & 0.2475 & 0.3250 & 0.0998 & 0.7383 & 0.5430 & 0.3769 & 0.2431 & 0.3070 & 0.4400 & 0.2895 & 0.3659 & 0.5364 \\
\midrule
PrDiMP50 \cite{2020Know}            & 0.2756      & 0.3218      & 0.2103 & 0.2822 & 0.3701 & 0.0 & 0.7149 & 0.5517 & 0.3841 & 0.0 & 0.3213 & 0.3764 & 0.3235 & 0.4612 & 0.4204 \\
DiMP50  \cite{bhat2019learning}     & 0.2579      & 0.3197      & 0.2953 & 0.2966 & 0.3914 & 0.0 & 0.6653 & 0.5249 & 0.3396 & 0.0 & 0.2548 & 0.5497 & 0.3090 & 0.4350 & 0.4284 \\
ATOM \cite{2019ATOM}                & 0.2072      & 0.2825      & 0.2737 & 0.2502 & 0.2703 & 0.0 & 0.6847 & 0.5148 & 0.2879 & 0.0 & 0.2817 & 0.5320 & 0.2319 & 0.3533 & 0.3084 \\
SiamRPN \cite{2018High}             & 0.1981      & 0.2269      & 0.3516 & 0.2418 & 0.2220 & 0.3709 & 0.6554 & 0.4944 & 0.3115 & 0.4398 & 0.2174 & 0.5574 & 0.2142 & 0.2855 & 0.4025 \\
D3S \cite{lukezic2020d3s}           & 0.1409      & 0.1983      & 0.2574 & 0.2035 & 0.1383 & 0.0 &  0.4988 & 0.4181 & 0.2446 & 0.0 & 0.2500 & 0.4180 & 0.1774 & 0.2547 & 0.2726 \\
SiamFC \cite{bertinetto2016fully}   & 0.0993      & 0.1617      & 0.1530 & 0.1174 & 0.0899 & 0.0 & 0.2795 & 0.3393 & 0.1529 & 0.0 & 0.1185 & 0.1839 & 0.1042 & 0.1774 & 0.2242 \\
\midrule
AlphaRef \cite{Kristan2020a}        & \bf{0.3765} & 0.3993      & 0.3430 & \textbf{0.3995} & 0.3761 & 0.0 & 0.7202 & 0.6087 & \textbf{0.4927} & 0.0 & 0.3437 & 0.4144 & 0.3725 & 0.3963 & 0.5496 \\
RPT \cite{Kristan2020a}             & 0.3008      & 0.3262      & 0.1889 & 0.3066 & 0.2769 & 0.4994 & 0.6034 & 0.5486 & 0.3673 & 0.4998 & 0.2997 & 0.4569 & 0.2976 & 0.3268 & 0.4945 \\
OceanPlus \cite{Kristan2020a}       & 0.2456      & 0.2971      & 0.2562 & 0.2298 & 0.2374 & 0.4993 & 0.6970 & 0.5276 & 0.3458 & 0.4998 & 0.2590 & 0.5353 & 0.2471 & 0.3185 & 0.4207 \\
\midrule
DeT-ATOM-MC                         & 0.316       & \bf{0.446}  & \bf{0.712} & 0.377 & 0.399 & 0.499 & 0.619 & 0.517 & 0.393 & 0.500 & 0.317 & 0.750 & 0.363 & 0.370 & 0.468 \\
DeT-ATOM-Max                        & 0.264       & 0.379       & 0.524      & 0.398 & 0.377 & 0.499 & 0.670 & 0.516 & 0.351 & 0.500 & 0.280  & 0.698 & 0.324 & 0.410 & 0.468\\
DeT-ATOM-Mean                       & 0.271       & 0.436       & 0.572      & 0.316 & 0.406 & 0.499 & 0.719 & 0.528 & 0.344 & 0.500 & 0.261  & 0.712 & 0.322 & 0.386 0.462 \\
DeT-DiMP50-MC                       & 0.378       & 0.486 & 0.691 & 0.468 & 0.481 & 0.499 & 0.738 & 0.550 & 0.483 & 0.500 & 0.320 & 0.718 & 0.413 & 0.414 & 0.521\\
DeT-DiMP50-Max                      & 0.424       & 0.471 & 0.739 & 0.496 & 0.505 & 0.499 & 0.638 & 0.646 & 0.501 & 0.500 & 0.298 & 0.729 & 0.463 & 0.482 & 0.550 \\
DeT-DiMP50-Mean                     & 0.398       & 0.458 & 0.719 & 0.456 & 0.469 & 0.499 & 0.760 & 0.654 & 0.505 & 0.500 & 0.314 & 0.723 & 0.431 & 0.464 & 0.537 \\
% Baseline   & - & - & - & LT & RGBD\\
\bottomrule
\end{tabularx}%
}
% \end{sidewaystable}
\end{center}
\end{table*}


==> tbl/tbl_fscores_over_sequence.tex <==
\newcolumntype{C}{>{\centering\arraybackslash}X}
\begin{table*}[t]
\begin{center}
\caption{
Optimal F-score averaged over overlap thresholds for the visual attributes on each sequence.
}
\label{tbl:fscores_attributes_on_DeTrack}
\resizebox{0.95\linewidth}{!}{%
% \begin{sidewaystable}
% \footnotesize
% \setlength\tabcolsep{3.6pt} % default value: 6pt
\begin{tabularx}{1.02\linewidth}{l | c c c | c c c}
\toprule
Sequence & \multicolumn{3}{c|}{DiMP50} & \multicolumn{3}{c}{DeT-DiMP50-Max} \\
\midrule
backpack\_blue                  & 0.616 & 0.647 & 0.631 &  0.679 & 0.690 & 0.685 \\
backpack\_robotarm\_lab\_occ    & 0.810 & 0.800 & 0.805 &  0.838 & 0.818 & 0.828 \\
backpack\_room\_noocc\_1        & 0.862 & 0.858 & 0.860 &  0.854 & 0.850 & 0.852 \\
bag\_outside                    & 0.636 & 0.685 & 0.660 &  0.426 & 0.459 & 0.442 \\
bicycle2\_outside               & 0.538 & 0.694 & 0.606 &  0.788 & 0.623 & 0.696 \\
bicycle\_outside                & 0.773 & 0.773 & 0.773 &  0.784 & 0.753 & 0.768 \\
bottle\_box                     & 0.318 & 0.390 & 0.350 &  0.281 & 0.394 & 0.328 \\
bottle\_room\_noocc\_1          & 0.117 & 0.117 & 0.117 &  0.731 & 0.731 & 0.730 \\
bottle\_room\_occ\_1            & 0.798 & 0.799 & 0.798 &  0.799 & 0.809 & 0.804 \\
box1\_outside                   & 0.201 & 0.175 & 0.187 &  0.649 & 0.643 & 0.646 \\
box\_darkroom\_noocc\_1         & 0.629 & 0.601 & 0.615 &  0.715 & 0.729 & 0.722 \\
box\_darkroom\_noocc\_10        & 0.390 & 0.390 & 0.390 &  0.492 & 0.492 & 0.492 \\
box\_darkroom\_noocc\_2         & 0.421 & 0.415 & 0.418 &  0.655 & 0.678 & 0.667 \\
box\_darkroom\_noocc\_3         & 0.566 & 0.579 & 0.573 &  0.748 & 0.757 & 0.752 \\
box\_darkroom\_noocc\_4         & 0.662 & 0.648 & 0.655 &  0.735 & 0.735 & 0.735 \\
box\_darkroom\_noocc\_5         & 0.375 & 0.384 & 0.379 &  0.801 & 0.795 & 0.798 \\
box\_darkroom\_noocc\_6         & 0.358 & 0.358 & 0.358 &  0.807 & 0.807 & 0.807 \\
box\_darkroom\_noocc\_7         & 0.293 & 0.293 & 0.293 &  0.662 & 0.630 & 0.645 \\
box\_darkroom\_noocc\_8         & 0.254 & 0.254 & 0.254 &  0.775 & 0.765 & 0.770 \\
box\_darkroom\_noocc\_9         & 0.273 & 0.273 & 0.273 &  0.638 & 0.638 & 0.638 \\
box\_room\_noocc\_1             & 0.395 & 0.395 & 0.395 &  0.751 & 0.693 & 0.721 \\
box\_room\_noocc\_2             & 0.267 & 0.267 & 0.267 &  0.440 & 0.440 & 0.440 \\
box\_room\_noocc\_3             & 0.107 & 0.107 & 0.107 &  0.256 & 0.256 & 0.256 \\
box\_room\_noocc\_4             & 0.787 & 0.787 & 0.787 &  0.780 & 0.787 & 0.787 \\ 
box\_room\_noocc\_5             & 0.783 & 0.783 & 0.783 &  0.595 & 0.590 & 0.592 \\
box\_room\_noocc\_6             & 0.611 & 0.593 & 0.602 &  0.838 & 0.838 & 0.838 \\
box\_room\_noocc\_7             & 0.742 & 0.742 & 0.742 &  0.828 & 0.828 & 0.828 \\ 
box\_room\_noocc\_8             & 0.795 & 0.700 & 0.744 &  0.754 & 0.754 & 0.754 \\ 
box\_room\_noocc\_9             & 0.724 & 0.165 & 0.268 &  0.832 & 0.189 & 0.309 \\ 
box\_room\_occ\_1               & 0.170 & 0.224 & 0.193 &  0.329 & 0.432 & 0.373 \\ 
box\_room\_occ\_2               & 0.495 & 0.524 & 0.509 &  0.790 & 0.769 & 0.779 \\ 
boxes\_backpack\_room\_occ\_1   & 0.698 & 0.697 & 0.697 &  0.672 & 0.653 & 0.662 \\
boxes\_humans\_room\_occ\_1     & 0.221 & 0.156 & 0.183 &  0.585 & 0.619 & 0.602 \\
boxes\_office\_occ\_1           & 0.356 & 0.347 & 0.352 &  0.720 & 0.737 & 0.352 \\ 
boxes\_room\_occ\_1             & 0.328 & 0.330 & 0.329 &  0.561 & 0.576 & 0.569 \\ 
cart\_room\_occ\_1              & 0.681 & 0.497 & 0.574 &  0.686 & 0.160 & 0.260 \\ 
cartman                         & 0.766 & 0.730 & 0.748 &  0.659 & 0.682 & 0.670 \\ 
cartman\_robotarm\_lab\_noocc   & 0.762 & 0.762 & 0.762 &  0.804 & 0.804 & 0.804 \\ 
case                            & 0.646 & 0.592 & 0.618 &  0.320 & 0.334 & 0.327 \\ 
container\_room\_noocc\_1       & 0.860 & 0.860 & 0.860 &  0.874 & 0.874 & 0.874 \\ 
dog\_outside                    & 0.812 & 0.812 & 0.812 &  0.809 & 0.809 & 0.809 \\ 
human\_entry\_occ\_1            & 0.766 & 0.778 & 0.772 &  0.709 & 0.712 & 0.711 \\ 
human\_entry\_occ\_2            & 0.772 & 0.739 & 0.755 &  0.754 & 0.700 & 0.726 \\
humans\_corridor\_occ\_1        & 0.313 & 0.385 & 0.345 &  0.322 & 0.372 & 0.345 \\ 
humans\_corridor\_occ\_2\_A     & 0.351 & 0.503 & 0.414 &  0.370 & 0.515 & 0.431 \\ 
humans\_corridor\_occ\_2\_B     & 0.673 & 0.742 & 0.706 &  0.613 & 0.695 & 0.651 \\ 
humans\_longcorridor\_staricase\_occ\_1 & 0.319 & 0.406 & 0.357 & 0.504 & 0.586 & 0.542 \\ 
humans\_shirts\_room\_occ\_1\_A & 0.712 & 0.723 & 0.718 & 0.742 & 0.746 & 0.744 \\ 
humans\_shirts\_room\_occ\_1\_B & 0.426 & 0.510 & 0.464 & 0.422 & 0.500 & 0.458 \\ 
jug                             & 0.449 & 0.470 & 0.459 & 0.559 & 0.559 & 0.559 \\ 
mug\_ankara                     & 0.733 & 0.726 & 0.729 & 0.743 & 0.736 & 0.739 \\ 
mug\_gs                         & 0.557 & 0.560 & 0.559 & 0.574 & 0.563 & 0.569 \\ 
paperpunch                      & 0.192 & 0.221 & 0.205 & 0.719 & 0.637 & 0.675 \\ 
person\_outside                 & 0.757 & 0.504 & 0.605 & 0.749 & 0.498 & 0.598 \\ 
robot\_corridor\_noocc\_1       & 0.826 & 0.824 & 0.825 & 0.811 & 0.810 & 0.811 \\ 
robot\_corridor\_occ\_1         & 0.730 & 0.723 & 0.726 & 0.719 & 0.713 & 0.716 \\ 
robot\_human\_corridor\_noocc\_1\_A & 0.650 & 0.650 & 0.650 & 0.658 & 0.658 & 0.658 \\ 
robot\_human\_corridor\_noocc\_1\_B & 0.548 & 0.548 & 0.548 & 0.518 & 0.518 & 0.518 \\ 
robot\_human\_corridor\_noocc\_2    & 0.669 & 0.712 & 0.690 & 0.598 & 0.636 & 0.616 \\ 
robot\_human\_corridor\_noocc\_3\_A & 0.441 & 0.437 & 0.439 & 0.576 & 0.577 & 0.577 \\ 
robot\_human\_corridor\_noocc\_3\_B & 0.512 & 0.521 & 0.517 & 0.525 & 0.534 & 0.529 \\ 
robot\_lab\_occ                & 0.819 & 0.818 & 0.819 & 0.443 & 0.267 & 0.333 \\ 
teapot                         & 0.826 & 0.825 & 0.826 & 0.842 & 0.841 & 0.841 \\ 
tennis\_ball                   & 0.662 & 0.520 & 0.583 & 0.696 & 0.627 & 0.660 \\ 
thermos\_office\_noocc\_1      & 0.423 & 0.415 & 0.419 & 0.686 & 0.652 & 0.669 \\ 
thermos\_office\_occ\_1        & 0.434 & 0.462 & 0.447 & 0.510 & 0.466 & 0.487 \\ 
toy\_office\_noocc\_1          & 0.784 & 0.784 & 0.784 & 0.707 & 0.707 & 0.707 \\ 
toy\_office\_occ\_1            & 0.793 & 0.766 & 0.780 & 0.805 & 0.788 & 0.796 \\ 
trashcan\_room\_occ\_1         & 0.652 & 0.660 & 0.656 & 0.175 & 0.232 & 0.200 \\ 
trashcans\_room\_occ\_1\_A     & 0.122 & 0.132 & 0.127 & 0.657 & 0.382 & 0.483 \\ 
trashcans\_room\_occ\_1\_B     & 0.619 & 0.615 & 0.617 & 0.629 & 0.560 & 0.592 \\ 
trendNetBag\_outside           & 0.612 & 0.686 & 0.647 & 0.803 & 0.731 & 0.765 \\ 
trendNet\_outside              & 0.300 & 0.324 & 0.311 & 0.433 & 0.469 & 0.450 \\ 
trophy\_outside                & 0.712 & 0.703 & 0.707 & 0.640 & 0.639 & 0.639 \\ 
trophy\_room\_noocc\_1         & 0.134 & 0.134 & 0.134 & 0.546 & 0.537 & 0.542 \\ 
trophy\_room\_occ\_1           & 0.693 & 0.755 & 0.723 & 0.725 & 0.782 & 0.753 \\ 
two\_mugs                      & 0.791 & 0.733 & 0.761 & 0.808 & 0.795 & 0.802 \\ 
two\_tennis\_balls             & 0.605 & 0.594 & 0.600 & 0.636 & 0.611 & 0.623 \\ 
XMG\_outside                   & 0.516 & 0.517 & 0.516 & 0.812 & 0.814 & 0.813 \\
\bottomrule

\end{tabularx}%
}
% \end{sidewaystable}
\end{center}
\end{table*}

